Deeper-GXX: Deepening Arbitrary GNNs

Recently, motivated by real applications, a major research direction in graph neural networks (GNNs) is to explore deeper structures. For instance, the graph connectivity is not always consistent with the label distribution (e.g., the closest neighbors of some nodes are not from the same category). In this case, GNNs need to stack more layers, in order to find the same categorical neighbors in a longer path for capturing the class-discriminative information. However, two major problems hinder the deeper GNNs to obtain satisfactory performance, i.e., vanishing gradient and over-smoothing. On one hand, stacking layers makes the neural network hard to train as the gradients of the first few layers vanish. Moreover, when simply addressing vanishing gradient in GNNs, we discover the shading neighbors effect (i.e., stacking layers inappropriately distorts the non-IID information of graphs and degrade the performance of GNNs). On the other hand, deeper GNNs aggregate much more information from common neighbors such that individual node representations share more overlapping features, which makes the final output representations not discriminative (i.e., overly smoothed). In this paper, for the first time, we address both problems to enable deeper GNNs, and propose Deeper-GXX, which consists of the Weight-Decaying Graph Residual Connection module (WDG-ResNet) and Topology-Guided Graph Contrastive Loss (TGCL). Extensive experiments on real-world data sets demonstrate that Deeper-GXX outperforms state-of-the-art deeper baselines.

==> Abstract.tex <==
\begin{abstract}
Recent years have witnessed the surge of big data in many real-world applications. For graph data, the size of the graphs has been growing at an unprecedented speed. Among others, graph neural networks (GNNs) have proven successful at modeling graphs. However, shallow GNNs tend to have sub-optimal performance dealing with large-scale graphs or graphs with missing features. Therefore, it is necessary to increase the depth (i.e., the number of layers) of GNNs to capture more latent knowledge of the input data.
On the other hand, including more layers in GNNs typically decreases their performance due to, e.g., vanishing gradient and oversmoothing. Existing methods (\eg, PairNorm and DropEdge) mainly focus on addressing oversmoothing, but they suffer from some drawbacks such as requiring hard-to-acquire knowledge or having large training randomness. In addition, these methods simply incorporate ResNet to address vanishing gradient. They ignore an important fact: by stacking more and more layers with ResNet architecture, the information collected from faraway neighbors becomes dominant, compared with the information collected from the 1-hop and 2-hop neighbors, thus resulting in severe performance degradation.
In this paper, we first go deep into the architecture of ResNet and analyze why ResNet is not best suited for deeper GNNs. Then we propose a new residual architecture to attenuate the negative impact caused by ResNet. To address the drawbacks of these existing methods, we introduce the Topology-guided Graph Contrastive Loss named \layer. It utilizes node topological information and pulls the connected node pairs closer via contrastive learning regularization to obtain discriminative node representations. Combining the new residual architecture with \layer, an end-to-end framework named \name\ is proposed towards deeper GNNs. The extensive experiments on real-world data sets demonstrate the effectiveness and efficiency of \name\ compared with state-of-the-art baselines.

%\lc{Prof. He, I have updated the abstract. Could you leave some comments regarding whether the motivation of TGCL is sufficient? A back-up version is hid in the following command, for your information.}

% In the real word, when the size of graph data is large and node features are inadequate, Graph Neural Networks (GNNs) requires to stack many more network layers for capturing useful latent hidden representation to maintain the performance. To make GNNs deeper, two problems need to be solved (i.e., vanishing gradient and oversmoothing). However, we found nascent solutions on both sides have drawbacks.
% First, to make GNNs trainable, many pioneering deep GNNs methods just apply ResNet to alleviate the vanishing gradient problem. Nevertheless, applying ResNet on non-i.i.d data like graphs will cause the \textit{Shading Neighbours Effect}, by which a node will gradually ignore its neighbours in the information propagation scheme of GNNs, thus leading to sub-optimal performance.
% Second, to make the final node representation discriminative, many regularization functions are proposed to alleviate oversmoothing issue. While, if not all, prevalent de-oversmoothing methods need hard-to-determine data-driven hyperparameters or rely on training randomness, which cause the representation learning process tricky.
% In this paper, we aim to deal with mentioned problems. We first design the \textit{Auto-weighted Graph Residual Connection}, which erases the shading neighbours effect when solving the vanishing gradient problem. Then, we design the \textit{Topology-guided Contrastive Loss}, which replaces the hard-to-determine hyperparameters and training randomness with the easy-accessible topology information of the input graph. In the end, these two are combined into an end-to-end model-agnostic deep framework, \name, which shows the overwhelming performance with state-of-the-art baselines.

\end{abstract}




% Graph neural networks (GNNs) integrate the comprehensive relation of graph data and the representation learning capability of neural networks, which is one of the most popular deep learning methods and achieves state-of-the-art performance in many applications, such as natural language processing and computer vision. In real-world scenarios, increasing the depth (i.e., the number of layers) of GNNs is sometimes necessary to capture more latent knowledge of the input data to mitigate the uncertainty caused by missing values. However, involving more complex structures and more parameters will decrease the performance of GNN models. One reason called oversmoothing is recently introduced but the relevant research remains nascent. In general, oversmoothing makes the final representations of nodes indiscriminative, thus deteriorating the node classification and link prediction performance.
% In this paper, we first survey the current de-oversmoothing methods and propose three major metrics to evaluate a de-oversmoothing method, i.e., constant divergence indicator, easy-to-determine divergence indicator, and model-agnostic strategy. Then, we propose the Topology-guided Graph Contrastive Layer, named \name, which is the first de-oversmoothing method maintaining all three mentioned metrics. With the contrastive learning manner, we provide the theoretical analysis of the effectiveness of the proposed \name. Last but not least, we design extensive experiments to illustrate the empirical performance of \name\ comparing with state-of-the-art baselines.


==> Preliminaries.tex <==
\section{Background}
As mentioned above, de-oversmoothing methods~\citep{DBLP:conf/iclr/KlicperaBG19, DBLP:conf/aaai/ChenLLLZS20, DBLP:conf/iclr/ZhaoA20, DBLP:conf/iclr/RongHXH20, DBLP:conf/icml/ChenWHDL20, DBLP:conf/kdd/LiuGJ20, DBLP:conf/nips/Zhou0LZCH20} share the same logic of keeping the divergence between node representations but differ in specific methodologies focusing on different merits. By taking the union of the metrics used in different state-of-the-arts, we get three metrics to evaluate a de-oversmoothing algorithm comprehensively.

There are three metrics as shown in Table~\ref{tb:four_metrics}, including constant divergence indicator, easy-to-determine divergence indicator, and model-agnostic de-oversmoothing strategy. Divergence indicator is indispensable for guiding the final node representation similarity based on the specified distance measurement. Several de-oversmoothing methods like \citep{DBLP:conf/iclr/KlicperaBG19, DBLP:conf/iclr/ZhaoA20, DBLP:conf/icml/ChenWHDL20, DBLP:conf/kdd/LiuGJ20} achieve the constant divergence indicator, which means the guidance is much more robust and not dependent on the training process of GNNs. However, to guide the node representation similarity reasonably, the divergence indicator is not that easy to be determined. For example, PairNorm~\citep{DBLP:conf/iclr/ZhaoA20} is proposed as a normalization layer to keep the divergence of node representation against the original node feature. Instead of adding this regularizer directly to the learning objective of GNN models, PairNorm takes an alternative by rescaling the learned node representations with a constant hyperparameter to keep the original node feature divergence. PairNorm achieves two metrics: constant divergence indicator (i.e., the constant hyperparameter) and model-agnostic strategy (i.e., PairNorm can be added on different GNN models as a layer). However, the selection of that constant hyperparameter heavily depends on the prior knowledge of the input graph data, which is hard to determine. (The discussion of other de-oversmoothing methods can be found in Section 5.)

As shown in Table~\ref{tb:four_metrics}, PairNorm is an effective de-oversmoothing method that maintains two metrics but needs prior knowledge to scale divergence between node pairs. While our proposed \name\ transfers this hard-to-acquire prior knowledge into the topology information of the input graph, where the divergence guidance between nodes is constant and easy to be determined. To be specific, our \name\ is the first de-oversmoothing method attempting to maintain these three metrics at the same time. In the next section, we formally introduce the proposed \name\ with theoretical proof for the model effectiveness. Moreover, we prove that the objective of PairNorm is just a special case of our \name, which shows the effectiveness of our \name\ from another perspective. 

\begin{table}[t]
\caption{Comparison of current de-oversmoothing methods}
\scalebox{0.87}{
\begin{tabular}{|l|c|c|c|}
\hline
     & \begin{tabular}[c]{@{}c@{}}Constant\\ Divergence Indicator\end{tabular} & \begin{tabular}[c]{@{}c@{}}Easy-to-Determine\\ Divergence Indicator\end{tabular}  & \begin{tabular}[c]{@{}c@{}}Model-Agnostic\\ Strategy\end{tabular} \\ \hline\hline
APPNP~\citep{DBLP:conf/iclr/KlicperaBG19} &Yes    &No   &Yes \\ \hline
MADReg + AdaEdge~\citep{DBLP:conf/aaai/ChenLLLZS20} &No    &Not Sure  &Yes \\ \hline
PairNorm~\citep{DBLP:conf/iclr/ZhaoA20}   &Yes    &No &Yes \\ \hline
DropEdge~\citep{DBLP:conf/iclr/RongHXH20}   &No    &No  &Yes \\ \hline
GCNII~\citep{DBLP:conf/icml/ChenWHDL20}&Yes    &Yes   &No \\ \hline
DAGNN~\citep{DBLP:conf/kdd/LiuGJ20}&Yes    &No    &Yes \\ \hline
DGN~\citep{DBLP:conf/nips/Zhou0LZCH20}  &No    &No   &Yes \\ \hline
\name\ (Our Method)  &Yes    &Yes  &Yes \\ \hline
\end{tabular}}
\label{tb:four_metrics}
\end{table}


==> algorithm_backup.tex <==
\section{Proposed Method}
Throughout the paper, we use regular letters to denote scalars (\eg, $\alpha$), boldface lowercase letters to denote vectors (\eg, $\bm{v}$), and boldface uppercase letters to denote matrices (\eg, $\bm{A}$). 
We formalize the graph mining problem in the context of undirected graph $G = (V,E)$, where $V$ consists of $n$ vertices, and $E$ consists of $m$ edges. 
We let $\bm{A} \in \mathbb{R}^{n\times n}$ denote the adjacency matrix, $\bm{X}\in \mathbb{R}^{n\times d}$ denote the feature matrix, $\bm{D} \in \mathbb{R}^{n\times n}$ denote the diagonal matrix of vertex degrees, and $\bm{I} \in \mathbb{R}^{n\times n}$ denote the identity matrix, where $d$ is the feature dimension. For ease explanation, we denote $V_i$ as node $i$, $Z_i$ as the embedding of node $i$ by any type of GNNs and $A_i$ as the adjacency vector for node $i$. $\mathcal{N}_i$ is a set that contains the neighbors of node $i$ and $\mathcal{\bar{N}}_i$ is complement set of $\mathcal{N}_i$, which contains the non-neighbor of node $i$.

The main idea of \name~ is to infer the relation of any pair of nodes based on the topological structure of graph. Specifically, we expect that the representations of two nodes are similar if their adjacency vector are close enough. Otherwise, their representations should be discriminative. Thus, we propose the topology-guided contrastive loss formulated as follows:
\begin{equation}
\begin{split}
        L &= - \E_{\bm{V_i} \sim V}\E_{\bm{V_j} \in \mathcal{N}_i} [ \log \frac{\sigma f(\bm{Z_i}, \bm{Z_j})}{\sigma f(\bm{Z_i}, \bm{Z_j}) + \sum_{\bm{V_k} \in \mathcal{\bar{N}}_i}  \gamma f(\bm{Z_i}, \bm{Z_k})} ] \\
        \sigma &= 1- dist(\bm{A_i}, \bm{A_j})/n, ~~\gamma= dist(\bm{A_i}, \bm{A_k})
\end{split}
\label{ls}
\end{equation}
where $f(\cdot)$ is a similarity function, \eg, $f(a, b)=\exp(\frac{a \cdot b}{\tau})$, $\tau$ is the temperature and $dist(\cdot)$ is a distance measurement function, \eg, hamming distance. The intuition of Eq.~\ref{ls} is that if $\bm{V_i}$ and $\bm{V_j}$ are neighbors, then the similarity of their representations should be as large as possible, while if $\bm{V_i}$ and $\bm{V_k}$ are two remote nodes (not connected in graph), the similarity of their representations should be as small as possible, and the magnitude of dissimilarity is determined by how many neighbors these two nodes share.

\subsection{Theoretical Analysis}
In this subsection, we provide the analysis regarding the properties of the proposed contrastive loss.
\begin{Lemma}
\label{lemma_s}
Given a neighbor node pair sampled from the graph $G = (V,E)$, \ie, nodes $\bm{V_i}$ and $\bm{V_j}$, we have $I(\bm{Z_i}, \bm{Z_j}) \geq -L + \E_{\bm{V_i} \sim V} \log(|\mathcal{\bar{N}}_i|)$, where $I(\bm{Z_i}, \bm{Z_j})$ is the mutual information between two representations of the node pair $\bm{V_i}$ and $\bm{V_j}$, and $L$ is the topology-guided contrastive loss weighted by hamming distance measurement.
\end{Lemma}
\textbf{Proof:}
\textit{
Following the theoretical analysis in~\cite{oord2018representation}, the optimal value of $f(\bm{Z_i}, \bm{Z_j})$ is given by $\frac{P(\bm{V_j}|\bm{V_i})}{P(\bm{V_j})}$.
Thus, the weighted supervised contrastive loss could be rewritten as follows:
\begin{equation}
    \notag
    \begin{split}
        L &= - \E_{\bm{V_i} \sim V}\E_{\bm{V_j} \in \mathcal{N}_i} [ \log \frac{\sigma f(\bm{Z_i}, \bm{Z_j})}{\sigma f(\bm{Z_i}, \bm{Z_j}) + \sum_{\bm{V_k} \in \mathcal{\bar{N}}_i} \gamma f(\bm{Z_i}, \bm{Z_k})} ] \\
        &=  \E_{\bm{V_i} \sim V}\E_{\bm{V_j} \in \mathcal{N}_i} [ \log \frac{\sigma f(\bm{Z_i}, \bm{Z_j}) + \sum_{\bm{V_k} \in \mathcal{\bar{N}}_i} \gamma f(\bm{Z_i}, \bm{Z_k})}{\sigma f(\bm{Z_i}, \bm{Z_j})} ] \\
        &=  \E_{\bm{V_i} \sim V}\E_{\bm{V_j} \in \mathcal{N}_i} [ \log \frac{\sigma \frac{P(\bm{Z_j}|\bm{Z_i})}{P(\bm{Z_j})} + \sum_{\bm{V_k} \in \mathcal{\bar{N}}_i} \gamma \frac{P(\bm{Z_k}|\bm{Z_i})}{P(\bm{Z_k})}}{\sigma \frac{P(\bm{Z_j}|\bm{Z_i})}{P(\bm{Z_j})}} ] \\
        &=  \E_{\bm{V_i} \sim V}\E_{\bm{V_j} \in \mathcal{N}_i} [ \log( 1 + \frac{P(\bm{Z_j})}{\sigma P(\bm{Z_j}|\bm{Z_i})} \sum_{\bm{V_k} \in \mathcal{\bar{N}}_i} \gamma \frac{P(\bm{Z_k}|\bm{Z_i})}{P(\bm{Z_k})})] \\
    \end{split}
\end{equation}
Since $(\bm{V_i}, \bm{V_k})$ is defined as a remote node pair, it means that at least these two nodes are not connected in the graph, \ie, $A(i,k)=A(k,i)=0$. Therefore, we have $\gamma=dist(\bm{A_i}, \bm{A_k}) \in [2,n] $ for all remote node pairs and $\sigma \in [\frac{2}{n}, 1]$ for all neighbor node pairs with hamming distance measurement, which leads to  $\frac{P(\bm{Z_j})}{\sigma P(\bm{Z_j}|\bm{Z_i})} \geq \frac{P(\bm{Z_j})}{P(\bm{Z_j}|\bm{Z_i})}$ and $\gamma \frac{P(\bm{Z_k}|\bm{Z_i})}{P(\bm{Z_k})} \geq \frac{P(\bm{Z_k}|\bm{Z_i})}{P(\bm{Z_k})}$.
Thus, we have
\begin{equation}
    \notag
    \begin{split}
        L &\geq  \E_{\bm{V_i} \sim V}\E_{\bm{V_j} \in \mathcal{N}_i} [ \log( 1 + \frac{P(\bm{Z_j})}{ P(\bm{Z_j}|\bm{Z_i})} \sum_{\bm{V_k} \in \mathcal{\bar{N}}_i} \frac{P(\bm{Z_k}|\bm{Z_i})}{P(\bm{Z_k})})] \\
        &\approx  \E_{\bm{V_i} \sim V}\E_{\bm{V_j} \in \mathcal{N}_i} [ \log( 1 + \frac{P(\bm{Z_j})}{ P(\bm{Z_j}|\bm{Z_i})}  (|\mathcal{\bar{N}}_i| \E_{V_k} \frac{P(\bm{Z_k}|\bm{Z_i})}{P(\bm{Z_k})})] \\
        &=  \E_{\bm{V_i} \sim V}\E_{\bm{V_j} \in \mathcal{N}_i} [ \log( 1 + \frac{P(\bm{Z_j})}{ P(\bm{Z_j}|\bm{Z_i})}  |\mathcal{\bar{N}}_i|)] \\
        &\geq  \E_{\bm{V_i} \sim V}\E_{\bm{V_j} \in \mathcal{N}_i} [ \log(\frac{P(\bm{Z_j})}{ P(\bm{Z_j}|\bm{Z_i})}) + \log(|\mathcal{\bar{N}}_i|)] \\
        &= - I(\bm{Z_i}, \bm{Z_j}) + \E_{\bm{V_i} \sim V} \log(|\mathcal{\bar{N}}_i|) \\
        % &= - I(\bm{Z_i}, \bm{Z_j}) + N \\ 
        % &= -\frac{\bm{1_{A_i(a)=A_j(a)}}}{n}I(\bm{V_j}, \bm{V_i}) + N \\
    \end{split}
\end{equation}
% where $|\mathcal{\bar{N}}_i|$ is the number of remote node pairs for node $i$.
Finally, we have $I(\bm{Z_i}, \bm{Z_j}) \geq -L + \E_{\bm{V_i} \sim V} \log(|\mathcal{\bar{N}}_i|)$, which completes the proof.} \\

Lemma~\ref{lemma_s} shows that the topology-guided contrastive loss for the graph is the lower bound of the mutual information between two representations of a neighbor node pair. Notice that $\E_{\bm{V_i} \sim V} \log(|\mathcal{\bar{N}}_i|)$ is the average logarithm of the number of unconnected edges for the nodes in the graph, which means that \name\ tends to be a better lower bound if imposed on a sparser graph.


\subsection{Special Case}
PairNorm~\cite{DBLP:conf/iclr/ZhaoA20} can be considered as a special case of our proposed framework. In ~\cite{DBLP:conf/iclr/ZhaoA20}, the authors aim to minimize the following equation:

\begin{align}
    \min \sum_{V_i\in V} \| \bm{Z}_i - \bm{X}_i\|^2 + \sum_{(i,j)\in E} \| \bm{Z}_i - \bm{Z}_j\|^2 - \sum_{(i,j)\not\in E} \| \bm{Z}_i - \bm{Z}_j\|^2 
\end{align}
where $\bm{Z}_i$ is the node embedding of node $i$ and $\bm{X}_i$ is the original feature of node $i$. In the equation above, the first term is the reconstruction error, the second term aims to minimize the difference between two representations of a neighbor pair, and the last term aims to maximize the difference between two representations of a remote pair.

Back to our formulation (Equation~\ref{ls}), if we set the weights for both neighbor pair and remote pair to 1, use only one remote pair for contrastive learning and define the similarity function as $f(\bm{Z}_i, \bm{Z}_j)=e^{-\|\bm{Z}_i -\bm{Z}_j\|^2}$, we could rewrite Equation~\ref{ls} as follow:

\begin{equation}
\begin{split}
        L &= - \E_{\bm{V_i} \sim V}\E_{\bm{V_j} \in \mathcal{N}_i} [ \log \frac{ f(\bm{Z_i}, \bm{Z_j})}{ f(\bm{Z_i}, \bm{Z_j}) +f(\bm{Z_i}, \bm{Z_k})} ] \\
        &= \E_{\bm{V_i} \sim V}\E_{\bm{V_j} \in \mathcal{N}_i} [ \log(1+ \frac{f(\bm{Z_i}, \bm{Z_k})}{ f(\bm{Z_i}, \bm{Z_j})}) ] \\
        &\approx \E_{\bm{V_i} \sim V}\E_{\bm{V_j} \in \mathcal{N}_i} [ \log(e^{-\|\bm{Z}_i -\bm{Z}_k\|^2}) - \log(e^{-\|\bm{Z}_i -\bm{Z}_j\|^2}) ] \\
        &= \E_{\bm{V_i} \sim V}\E_{\bm{V_j} \in \mathcal{N}_i} [\|\bm{Z}_i -\bm{Z}_j\|^2  -\|\bm{Z}_i -\bm{Z}_k\|^2 ]\\
        % &= \frac{1}{|E|}[\sum_{(i,j)\in E} \| \bm{Z}_i - \bm{Z}_j\|^2 - \sum_{(i,j) \not\in E} \| \bm{Z}_i - \bm{Z}_j\|^2 ]
\end{split}
\label{ls2}
\end{equation}
We could see that Equation~\ref{ls2} is two regularization terms of PairNorm~\cite{DBLP:conf/iclr/ZhaoA20} except for the reconstruction error. Notice that PairNorm sets the weights for both neighbor pair and remote pair to be 1. This means that PairNorm only considers the first-order neighbor information of each node pair and ignores the topological structure information of the graph itself, which may lead to suboptimal performance. However, \name~ utilizes the similarity of two adjacency vectors of each node pair to embed the global topological structure information into the representation of each node such that GNNs can derive better discriminative representations for all nodes.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

